Boosting Novel Category Discovery Over Domains with Soft Contrastive Learning and All-in-One Classifier

Unsupervised domain adaptation (UDA) has proven to be highly effective in transferring knowledge from a label-rich source domain to a label-scarce target domain. However, the presence of additional novel categories in the target domain has led to the development of open-set domain adaptation (ODA) and universal domain adaptation (UNDA). Existing ODA and UNDA methods treat all novel categories as a single, unified unknown class and attempt to detect it during training. However, we found that domain variance can lead to more significant view-noise in unsupervised data augmentation, which affects the effectiveness of contrastive learning (CL) and causes the model to be overconfident in novel category discovery. To address these issues, a framework named Soft-contrastive All-in-one Network (SAN) is proposed for ODA and UNDA tasks. SAN includes a novel data-augmentation-based soft contrastive learning (SCL) loss to fine-tune the backbone for feature transfer and a more human-intuitive classifier to improve new class discovery capability. The SCL loss weakens the adverse effects of the data augmentation view-noise problem which is amplified in domain transfer tasks. The All-in-One (AIO) classifier overcomes the overconfidence problem of current mainstream closed-set and open-set classifiers. Visualization and ablation experiments demonstrate the effectiveness of the proposed innovations. Furthermore, extensive experiment results on ODA and UNDA show that SAN outperforms existing state-of-the-art methods.

==> tab_oda_copy.tex <==
      

\begin{minipage}[t]{\textwidth}
  \begin{minipage}[t]{0.63\textwidth}
    \makeatletter\def\@captype{table}
    \begin{tabular}{l|p{14pt}p{14pt}p{14pt}p{14pt}p{14pt}p{18pt}|p{14pt}}
      \toprule
      \multirow{2}{*}{Method} & \multicolumn{6}{c|}{Office (10 / 0 / 11)} & \multirow{2}{*}{Avg}                                                             \\
                              & A2D                                       & A2W                  & D2A       & D2W       & W2D       & W2A       &           \\\hline
      UAN                     & 38.9                                      & 46.8                 & 68.0      & 68.8      & 53.0      & 54.9      & 55.1      \\
      CMU                     & 52.6                                      & 55.7                 & 76.5      & 75.9      & 64.7      & 65.8      & 73.1      \\
      DANCE                   & 84.9                                      & 78.8                 & 79.1      & 78.8      & 88.9      & 68.3      & 79.8      \\
      DCC                     & 58.3                                      & 54.8                 & 67.2      & 89.4      & 80.9      & 85.3      & 72.6      \\
      ROS                     & 82.4                                      & 82.1                 & 77.9      & 96.0      & 99.7      & 77.2      & 85.9      \\
      USFDA                   & 85.5                                      & \bf{79.8}            & \bf{83.2} & 90.6      & 88.7      & 81.2      & 84.8      \\
      OVANet                  & 90.5                                      & 88.3                 & 86.7      & 98.2      & 98.4      & 88.3      & 91.7      \\
      GATE                    & 88.4                                      & 86.5                 & 84.2      & 95.0      & 96.7      & 86.1      & 89.5      \\ \hline
      \ours                   & \bf{90.5}                                 & \bf{93.5}            & \bf{91.7} & \bf{98.9} & \bf{99.9} & \bf{92.8} & \bf{94.6} \\
      \ours$^*$               & \bf{90.5}                                 & \bf{93.5}            & \bf{91.7} & \bf{98.9} & \bf{99.9} & \bf{92.8} & \bf{94.6} \\
      \toprule
      % \bottomrule[1.5pt]
    \end{tabular}
    \vspace{-4mm}
    \caption{\textbf{H-score of Office datasets in the open-partial DA setting.}}
  \label{tb_office_oda}
  \end{minipage}
  \begin{minipage}[t]{0.35\textwidth}
    \makeatletter\def\@captype{table}
    \begin{tabular}{l|c|c}
      \toprule
      \multirow{2}{*}{Method} & VisDA       & VisDA       \\
                              & ODA         & OPDA        \\
                              & (6 / 0 / 6) & (6 / 3 / 3) \\\hline
      UAN                     & 51.9        & 30.5        \\
      CMU                     & 54.2        & 34.6        \\
      DANCE                   & 67.5        & 42.8        \\
      DCC                     & 59.6        & 43.0        \\
      OVANet                  & 66.1        & 53.1        \\
      GATE                    & 70.8        & 56.4        \\ \hline
      \ours                   & \bf{72.0}   & \bf{60.1}   \\
      \bottomrule
    \end{tabular}
    \vspace{-3mm}
    \caption{\textbf{H-score of VisDA datasets on open-partial DA and open DA setting.} }
    \label{tb_VisDA_opda_oda}
  \end{minipage}
\end{minipage}




